Uniform Forward-Modeling Analysis of Ultracool Dwarfs. III. Late-M and L Dwarfs in Young Moving Groups, the Pleiades, and the Hyades

We present a uniform forward-modeling analysis of 90 late-M and L dwarfs in nearby young (~$10-200$ Myr) moving groups, the Pleiades, and the Hyades using low-resolution ($R\approx150$) near-infrared ($0.9-2.4$ $\mathrm{\mu m}$) spectra and the BT-Settl model atmospheres. We derive the objects' effective temperatures, surface gravities, radii, and masses by comparing our spectra to the models using a Bayesian framework with nested sampling and calculate the same parameters using evolutionary models. Assuming the evolutionary-based parameters are more robust, our spectroscopically inferred parameters from BT-Settl exhibit two types of systematic behavior for objects near the M-L spectral type boundary. Several are clustered around $T_\mathrm{eff} \approx 1800$ K and $\log g\approx5.5$ dex, implying impossibly large masses ($150-1400$ $M_\mathrm{Jup}$), while others are clustered around $T_\mathrm{eff}\gtrsim3000$ K and $\log g\lesssim3.0$ dex, implying non-physical low masses and unreasonably young ages. We find the fitted BT-Settl model spectra tend to overpredict the peak $J$ and $H$-band flux for objects located near the M-L boundary, suggesting the dust content included in the model atmospheres is insufficient to match the observations. By adding an interstellar medium-like reddening law to the BT-Settl model spectra, we find the fits between models and observed spectra are greatly improved, with the largest reddening coefficients occurring at the M-L transition. This work delivers a systematic examination of the BT-Settl model atmospheres and constitutes the largest spectral analysis of benchmark late-M and L-type brown dwarfs to date.

==> spex.tex <==
\startlongtable
\centerwidetable
\begin{longrotatetable}
\begin{deluxetable}{lllcccr}
\tablecaption{IRTF/SpeX Observing Log}
\tabletypesize{\footnotesize}
\rotate
\tablewidth{0pt}
\tablehead{
  \colhead{Object} &
  \colhead{SIMBAD name} &
  \colhead{Discovery Ref} &
  \colhead{Obs Date (UT)} &
  \colhead{Slit (\arcsec)} &
  \colhead{$<$Airmass$>$} &  % \colhead{$\sec z$} &
  \colhead{$T_{int}$ (s)} 
  % \colhead{File} &
  % \colhead{RA/Spex} &
  % \colhead{DEC/Spex} &
  % \colhead{RA/Spex (degs)} &
  % \colhead{DEC/Spex (degs)} &
  % \colhead{Grat} &
  % \colhead{$R$} &
  % \colhead{$N_{exp} \times t$ (s)} &
  % \colhead{$<S/N> (Y,J,H,H_{blue},K,K_{blue})$} 
}

\startdata
% SPEX_SUMMARIZE.PRO: Sat Aug  6 15:55:11 2022 mliu@Mike-Liu-2021-Macbook-Pro.local 
% infile = "list.spectra"
% 
% Note: Coordinates from IRTF image headers are not very accurate, can be off by several arcsec
% 
% Object                     & SIMBAD name                    &  Discovery Ref                       & Date(UT)    &  Slit (") &   AM   &  Tint(s)   % File                           &   RA_Spex       & DEC_Spex      & RA_Sp(degs) & DEC_Sp(degs) &   N x Itime &  <SNR(Y,J,H,H_blue,K,K_blue)> \\
%
%----------------------------------------%
\cutinhead{Pleiades Members}
%----------------------------------------%
MHObd3                       & Cl$\ast$ Melotte 22 MHOBD 3    &  Stau98b                             & 2010-03-03  &  0.8\arcsec & 1.62 &   1320  \\ % MHOBD3_prz.fits                &   +03:41:54.05  & +23:05:11.7   &   55.475208 &   23.086583  &   11_x_120.0 &  39,  65,  41,  38,  41,  42, \\
UGCS J034334.48+255730.5     & UGCS J034334.48+255730.5       &  Lodi12a                             & 2010-03-03  &  0.8\arcsec & 1.15 &    960  \\ % UGCS-PL-12_prz.fits            &   +03:46:48.01  & +23:10:06.3   &   56.700042 &   23.168417  &    8_x_120.0 &  65,  97,  79,  67,  71,  78, \\  % note: file name is wrong, this object is UGCS-PL-15
%UGCS-PL-12                  & UGCS J034334.48+255730.5       &  Lodi12a                             & 2010-03-03  &  0.8\arcsec & 1.15 &    960  \\ % UGCS-PL-12_prz.fits            &   +03:46:48.01  & +23:10:06.3   &   56.700042 &   23.168417  &    8_x_120.0 &  65,  97,  79,  67,  71,  78, \\  % note: file name is wrong, this object is UGCS-PL-15
Roque 7                      & Cl$\ast$ Melotte 22 PLIZ 16    &  Bouv98                              & 2010-03-01  &  0.8\arcsec & 1.25 &   1320  \\ % Roque7_prz.fits                &   +03:43:39.88  & +24:30:18.2   &   55.916167 &   24.505056  &   11_x_120.0 &  36,  55,  34,  31,  38,  38, \\
BRB 4                        & Cl$\ast$ Melotte 22 BRB 4      &  Biha06                              & 2010-03-01  &  0.8\arcsec & 2.02 &    600  \\ % BRB4_prz.fits                  &   +03:44:23.34  & +25:38:50.4   &   56.097250 &   25.647333  &    5_x_120.0 & 125, 192, 112, 104, 105, 109, \\
BRB 27                       & Cl$\ast$ Melotte 22 PLIZ 1262  &  Bouy06a;Biha06                      & 2008-12-02  &  0.8\arcsec & 1.15 &   3060  \\ % BRB27.fits                     &   +03:44:27.57  & +25:44:46.2   &   56.114875 &   25.746167  &   17_x_180.0 &   5,  15,  12,  11,  16,  16, \\
PLZJ 61                      & Cl$\ast$ Melotte 22 PLIZ 2141  &  Biha06                              & 2009-09-29  &  0.8\arcsec & 1.05 &   5040  \\ % PLZJ61_prz.fits                &   +03:44:30.81  & +25:35:17.4   &   56.128375 &   25.588167  &   28_x_180.0 &  19,  46,  37,  35,  36,  40, \\
SI2M-10                      & Cl$\ast$ Melotte 22 SHF 10     &  Stau07                              & 2010-03-02  &  0.8\arcsec & 2.04 &    840  \\ % SI2M-10_prz.fits               &   +03:45:38.73  & +23:43:58.6   &   56.411375 &   23.732944  &    7_x_120.0 & 103, 156,  94,  86,  85,  87, \\
SI2M-16                      & Cl$\ast$ Melotte 22 SHF 16     &  Stau07                              & 2009-10-31  &  0.8\arcsec & 1.42 &   1080  \\ % SI2M-16.fits                   &   +03:45:49.87  & +23:57:04.9   &   56.457792 &   23.951361  &    9_x_120.0 &  71,  99,  91,  89,  62,  69, \\
Roque 13                     & Cl$\ast$ Melotte 22 BPL 79     &  Zapa97                              & 2009-10-30  &  0.8\arcsec & 1.28 &   1980  \\ % ROQUE_13.fits                  &   +03:45:50.46  & +24:09:01.3   &   56.460250 &   24.150361  &   11_x_180.0 &  41,  66,  74,  65,  42,  46, \\
SI2M-37                      & Cl$\ast$ Melotte 22 SHF 37     &  Stau07                              & 2010-03-02  &  0.8\arcsec & 1.47 &   1800  \\ % SI2M-42_prz.fits               &   +03:46:49.84  & +24:00:29.0   &   56.707667 &   24.008056  &   15_x_120.0 &  57,  95,  58,  55,  53,  57, \\
Teide 1                      & Cl$\ast$ Melotte 22 TEIDE 1    &  Rebo95                              & 2009-10-29  &  0.8\arcsec & 1.32 &   1980  \\ % Teide1.fits                    &   +03:47:18.51  & +24:22:33.3   &   56.827125 &   24.375917  &   11_x_180.0 &  47,  72,  57,  51,  40,  45, \\
CFHT-PL-11                   & Cl$\ast$ Melotte 22 BPL 152    &  Zapa97                              & 2010-03-02  &  0.8\arcsec & 1.11 &   1320  \\ % CFHT-PL11_prz.fits             &   +03:47:38.33  & +24:36:29.6   &   56.909708 &   24.608222  &   11_x_120.0 &  57,  87,  58,  52,  51,  56, \\
UGCS J034815.64+255008.9     & UGCS J034815.64+255008.9       &  Lodi12a;Zapa14                      & 2009-10-29  &  0.8\arcsec & 1.03 &   7020  \\ % Lodieu_x1.fits                &    +03:48:16.01  & +25:50:19.6   &   57.066708 &   25.838778   &  39_x_180.0 &   5,  19,  18,  15,  14,  16, \\
Roque 25                     & Cl$\ast$ Melotte 22 ROQUE 25   &  Mart98c                             & 2009-09-30  &  0.8\arcsec & 1.04 &   6480  \\ % Roque25_prz.fits               &   +03:48:30.37  & +22:44:51.6   &   57.126542 &   22.747667  &   36_x_180.0 &  24,  52,  41,  38,  41,  43, \\
CFHT-PL-5                    & Cl$\ast$ Melotte 22 CFHT 5     &  Bouv98                              & 2010-03-01  &  0.8\arcsec & 1.11 &   1320  \\ % CFHT-PL5_prz.fits              &   +03:48:44.11  & +24:37:28.9   &   57.183792 &   24.624694  &   11_x_120.0 & 111, 146,  93,  87,  84,  89, \\
HHJ 3                        & Cl$\ast$ Melotte 22 HHJ 3      &  Hamb93                              & 2009-11-03  &  0.8\arcsec & 1.07 &   2040  \\ % HHJ3_0.8prism_2009nov03.fits   &   +03:48:50.20  & +22:44:33.5   &   57.209167 &   22.742639  &   17_x_120.0 &  56,  93,  83,  79,  62,  66, \\
SI2M-54                      & Cl$\ast$ Melotte 22 HHJ 8      &  Hamb93                              & 2009-10-31  &  0.8\arcsec & 1.21 &   2040  \\ % SI2M-54.fits                   &   +03:48:55.48  & +24:21:40.6   &   57.231167 &   24.361278  &   17_x_120.0 &  95, 139, 135, 120,  80,  98, \\
PLZJ 21                      & Cl$\ast$ Melotte 22 PLIZ 31    &  Mora03                              & 2009-10-29  &  0.8\arcsec & 1.44 &   3060  \\ % PLZJ-21.fits                   &   +03:51:47.44  & +24:40:09.3   &   57.947667 &   24.669250  &   17_x_180.0 &  13,  25,  22,  18,  17,  19, \\
Teide 2                      & Cl$\ast$ Melotte 22 PLIZ 3     &  Mart98e                             & 2009-10-31  &  0.8\arcsec & 1.09 &   1560  \\ % Teide2.fits                    &   +03:52:06.98  & +24:16:00.8   &   58.029083 &   24.266889  &   13_x_120.0 &  64,  89,  75,  71,  48,  55, \\
PLZJ 10                      & Cl$\ast$ Melotte 22 PLIZ 35    &  Bouv98                              & 2009-10-30  &  0.8\arcsec & 1.02 &   7380  \\ % Lodieu_x3.fits                 &   +03:52:39.42  & +24:46:28.5   &   58.164250 &   24.774583  &   41_x_180.0 &  15,  33,  33,  30,  24,  27, \\
CFHT-PL-25                   & Cl$\ast$ Melotte 22 PLIZ 20    &  Bouv98                              & 2009-10-29  &  0.8\arcsec & 1.12 &   3780  \\ % CFHT-Pl-25.fits                &   +03:54:05.81  & +23:34:03.1   &   58.524208 &   23.567528  &   21_x_180.0 &  29,  64,  48,  42,  32,  36, \\
PLZJ 4                       & Cl$\ast$ Melotte 22 BRB 21     &  Biha06                              & 2009-10-01  &  0.8\arcsec & 1.04 &   8460  \\ % PLZJ4_prz.fits                 &   +03:54:09.82  & +23:41:40.5   &   58.540917 &   23.694583  &   47_x_180.0 &  18,  45,  42,  40,  40,  43, \\
PLZJ 77                      & Cl$\ast$ Melotte 22 PLIZ 28    &  Mora03                              & 2009-10-31  &  0.8\arcsec & 1.03 &   6600  \\ % PLZJ-77.fits                   &   +03:54:14.06  & +23:17:55.1   &   58.558583 &   23.298639  &   55_x_120.0 &  15,  34,  31,  27,  24,  27, \\
%----------------------------------------%
\cutinhead{Refuted Pleiades Members}
%----------------------------------------%
SI2M-28                      & Cl$\ast$ Melotte 22 SHF 28     &  Stau07                              & 2010-03-03  &  0.8\arcsec & 2.06 &   1320  \\ % SI2M-28_prz.fits               &   +03:46:18.57  & +23:48:53.8   &   56.577375 &   23.814944  &   11_x_120.0 &  22,  37,  26,  24,  25,  25, \\
CFHT-PL-6                    & Cl$\ast$ Melotte 22 CFHT 6     &  Bouv98                              & 2009-10-31  &  0.8\arcsec & 1.24 &    720  \\ % CFHT-Pl-6.fits                 &   +03:52:07.49  & +23:59:14.3   &   58.031208 &   23.987306  &    6_x_120.0 &  69,  90,  85,  95,  56,  61, \\
CFHT-PL-15                   & Cl$\ast$ Melotte 22 BRB 13     &  Bouv98                              & 2009-10-30  &  0.8\arcsec & 1.10 &   1980  \\ % CFHT-Pl-15.fits                &   +03:55:13.04  & +23:17:36.6   &   58.804333 &   23.293500  &   11_x_180.0 &  40,  59,  65,  62,  36,  43, \\
%----------------------------------------%
\cutinhead{Field Objects}
% ----------------------------------------%
% SPEX_SUMMARIZE.PRO: Thu Sep 15 16:09:46 2022 mliu@sdhcp103.ifa.hawaii.edu 
% infile = "list.spectra-other"
%
% Object                     &                                &                                      & Date(UT)    &  Slit (")   &   AM &  Tint(s)   \\  % File                                       &   RA_Spex       & DEC_Spex      & RA_Sp(degs) & DEC_Sp(degs &    N x Itime &  <SNR(Y,J,H,H_blue,K,K_blue)> \\
2MASS J00192626+4614078      &   PM J00194+4614               & Cruz03                               & 2015-07-15  &  0.5\arcsec & 1.12 &     88   \\  % 2MASSJ0019+4614_0.5prism_2015jul15.fits    &              0  &            0  &  -99.000000 &  -99.000000 &    9_x_9.7   &    86, 161, 175, 172, 132, 134, \\
TVLM 831-154910              &   TVLM 831-154910              & Tinn93d                              & 2014-10-15  &  0.8\arcsec & 1.08 &    208   \\  % TVLM831-154910_0.8prism_2014oct15.fits     &              0  &            0  &  -99.000000 &  -99.000000 &    7_x_29.7  &   139, 133, 117, 125,  72,  80, \\
PSO J058.0039+41.7950        &   \nodata                      & this work, Alle16b                   & 2016-03-22  &  0.5\arcsec & 1.31 &    777   \\  % YUF-29133-55877_0.5prism_2016mar22.fits    &              0  &            0  &  -99.000000 &  -99.000000 &   13_x_59.8  &    89, 157, 148, 127, 157, 159, \\
2MASS J04203904+2355502      &   2MASS J04203904+2355502      & Luhm06b                              & 2015-12-24  &  0.5\arcsec & 1.04 &    386   \\  % YU2-22006-39149_0.5prism_2015dec24.fits    &              0  &            0  &  -99.000000 &  -99.000000 &   13_x_29.7  &    28,  55,  51,  45,  50,  50, \\
Hya04                        &   2MASS J04421852+1754378      & Lodi14b                              & 2016-02-03  &  0.5\arcsec & 1.27 &   1076   \\  % Hya04_0.5prism_2016feb03.fits              &              0  &            0  &  -99.000000 &  -99.000000 &    9_x_119.5 &    39,  57,  39,  36,  42,  42, \\
2MASS J05445741+3705039      &   2MASS J05445741+3705039      & this work, Alle16b, Smit14b, Gagn18c & 2015-10-14  &  0.5\arcsec & 1.09 &    133   \\  % pm-L05-2015-10_0.5prism_2015oct14.fits     &              0  &            0  &  -99.000000 &  -99.000000 &    9_x_14.8  &    34,  93, 117, 107, 105, 107, \\
SSSPM J1102-3431             &   TWA 28                       & Scho05a                              & 2016-02-03  &  0.5\arcsec & 1.72 &    777   \\  % TWA28_0.5prism_2016feb03.fits              &              0  &            0  &  -99.000000 &  -99.000000 &   13_x_59.8  &   174, 207, 167, 157, 111, 118, \\
PSO J243.9421+67.2075        &   \nodata                      & this work                            & 2013-09-23  &  0.8\arcsec & 1.83 &    240   \\  % veryred-1527_0.8prism_2013sep23.fits       &   +16:15:45.82  & +67:12:36.0   &  243.940917 &   67.210000 &    2_x_120.0 &    10,  27,  30,  24,  53,  55, \\
PSO J316.1306$-$09.6562      &   2MASS J21043128-0939217      & this work, Alle16b, Gagn18c          & 2015-11-28  &  0.5\arcsec & 1.29 &    837   \\  % YU2-644-102045_0.5prism_2015nov28.fits     &              0  &            0  &  -99.000000 &  -99.000000 &    7_x_119.5 &    27,  41,  30,  25,  33,  35, \\
PSO J318.4243+35.1277        &   PSO J318.4243+35.1277        & Alle16                               & 2013-09-22  &  0.5\arcsec & 1.10 &     60   \\  % YMG-HS-6359-53211_0.5prism_2013sep22.fits  &   +21:13:41.76  & +35:07:44.7   &  318.424000 &   35.129083 &    2_x_30.0  &    53, 117, 100,  95,  83,  85, \\
WISEA J235422.31$-$081129.7  &   2MASS J23542220-0811289      & Schn17                               & 2013-09-22  &  0.8\arcsec & 1.14 &    240   \\  % veryred-2068_0.8prism_2013sep22.fits       &   +23:54:22.92  & -08:11:28.0   &  358.595500 &   -8.191111 &    2_x_120.0 &    13,  37,  39,  33,  46,  46, \\
\enddata


\tablerefs{Alle16 = \citet{2016ApJ...821..120A},
  Alle16b = \citet{2016PhDT.......189A},
  Biha06 = \citet{2006AA...458..805B},   %  Biha06 = \citet{2006A&A...458..805B},
  Bouv98 = \citet{1998AA...336..490B},   %  Bouv98 = \citet{1998A&A...336..490B},
  Bouy06a = \citet{2006ApJ...637.1056B},
  Cruz03 = \citet{2003AJ....126.2421C},
  Gagn18c = \citet{2018ApJ...862..138G},
  Hamb93 = \citet{1993AAS..100..607H},   %  Hamb93 = \citet{1993A&AS..100..607H},
  Lodi12a = \citet{2012MNRAS.422.1495L},
  Lodi14b = \citet{2014MNRAS.445.3908L},
  Luhm06b = \citet{2006ApJ...645..676L},
  Mart98c = \citet{1998ApJ...507L..41M},
  Mart98e = \citet{1998ApJ...499L..61M},
  Mora03 = \citet{2003AA...400..891M},   %  Mora03 = \citet{2003A&A...400..891M},
  Rebo95 = \citet{1995Natur.377..129R},
  Schn17 = \citet{2017AJ....153..196S},
  Scho05a = \citet{2005AA...430L..49S},  %  Scho05a = \citet{2005A&A...430L..49S},
  Smit14b = \citet{2014MNRAS.443.2327S},
  Stau98b = \citet{1998ApJ...504..805S},
  Stau07 = \citet{2007ApJS..172..663S},
  Tinn93d = \citet{1993ApJ...414..279T},
  Zapa97 = \citet{1997ApJ...491L..81Z},
  Zapa14 = \citet{2014AA...568A..77Z}.   %  Zapa14 = \citet{2014A&A...568A..77Z}.
}


% \tablecomments{The last column gives the median S/N of the spectrum for the standard IR bandpasses
%   and also for two wavelength regions free of methane absorption
%   ($H_{blue}$ = 1.49--1.63~\micron\ and $K_{blue}$ = 2.03--2.20~\micron).}

\end{deluxetable}
\end{longrotatetable}
